TLS 1.3 for engineers: An exploration of the TLS 1.3 specification and OpenJDK's Java implementation

The Internet delivered in excess of forty terabytes per second in 2017 (Cisco, 2018), and over half of today's Internet traffic is encrypted (Sandvine, 2018); enabling trade worth trillions of dollars (Statista, 2017). Yet, the underlying encryption technology is only understood by a select few. This manuscript broadens understanding by exploring TLS, an encryption technology used to protect application layer communication (including HTTP, FTP and SMTP traffic), and by examining Oracle's Java implementation. We focus on the most recent TLS release, namely, version 1.3, which is defined by RFC 8446.

==> abstract.tex <==
\begin{abstract}
\textcolor{red}{...TO DO...}
\end{abstract}


==> preface.tex <==
\section*{Preface}



==> specification.tex <==
\newcommand{\genericType}{\texttt{T}}

\newcommand{\TLSPrimitiveType}[1]{\textsf{#1}}

\newcommand{\uint}{\TLSPrimitiveType{uint8}}
\newcommand{\uintSixteen}{\TLSPrimitiveType{uint16}}
\newcommand{\uintTwentyFour}{\TLSPrimitiveType{uint24}}
\newcommand{\uintThirtyTwo}{\TLSPrimitiveType{uint32}}
\newcommand{\uintSixtyFour}{\TLSPrimitiveType{uint64}}
\newcommand{\opaque}{\TLSPrimitiveType{opaque}}

\newcommand{\struct}{\TLSPrimitiveType{struct}}
\newcommand{\genericField}{f}

\section{Specification}\label{sec:specification}

\textcolor{blue}{This appendix includes code listings from RFC 8446.  
  If they are used, then the necessary license should be included.}

\textcolor{red}{Recalling formal syntax doesn't seem particularly useful;
  readers can refer to the RFC. Drop this appendix?}
 

\marginpar{There are perhaps better ways to present the syntax.}

This appendix recalls specifications for \ClientHello\ (Listing~\ref{lst:ClientHello})
and \ServerHello\ (Listing~\ref{lst:ServerHello}) messages. Those specifications 
are stated using the following syntax: Basic type 
%
  \uint\
%
is defined as an unsigned 8 bit integer. Types can be aliased and 
%
  \genericType\ \genericType'\ 
%
denotes aliasing type \genericType\ as new type \genericType'. 
For readability, a single byte containing uninterpreted 
data is aliased:
%
  \uint\ \opaque.
%
Multi-byte types can be derived by concatenation and
%
  \genericType\ \genericType'[n]
%
denotes a new type \genericType' that is an $n$-byte 
vector of type \genericType, under the constraint that 
$n$ is a multiple of the size of \genericType. Hence, 16, 
24, 32, and 32 bit unsigned integers are introduced as follows:
%
  \uint\ \uintSixteen[2];
  \uint\ \uintTwentyFour[3];
  \uint\ \uintThirtyTwo[4];
  \uint\ \uintSixtyFour[8].
%
Variable-length vectors are denoted
%
  \genericType\ \genericType'\textless{}floor..ceiling\textgreater{},
%
where `floor' and `ceiling' define lower and upper byte
bounds, under the constraint that they are multiples of 
the size of \genericType.
Data of variable-length is prepended with the data's
actual length when streamed.
%%
%%
%%
Structured types may be constructed from primitives types and 
%
  \struct~\{ \genericType1 \genericField1; \genericType2 \genericField2; ...; \genericType{}n \genericField{}n~\} \genericType\
%
denotes a structured type \genericType\ containing 
field \genericField1 of type \genericType1, 
field \genericField2 of type \genericType2, and 
similarly for \genericField3,\genericType3, ..., \genericField{}n,\genericType{}n. 
Fields may be assigned a fixed value using ``='', e.g., 
%
\struct~\{ 
  \genericType\ \genericField\ = 8; 
  \genericType' \genericField'~\} 
\genericType\ 
%
assigns 8 to \genericType.\genericField.


\lstinputlisting[
  float=t,
  linerange={
    1541-1553,%ClientHello
    1915-1919%Extension
  },
  label=lst:ClientHello,
  caption={[\ClientHello\ specification]
    \ClientHello\ specification, which aliases type 
    \TLSProtocolVersion\ as a 16 bit unsigned integer (Line~1541), 
    \TLSRandom\ as a 32 byte unsigned integer (Line~1542), and 
    \TLSCipherSuite\ as a 2 byte integer (Line~1544),
    and defines structured type \ClientHello\ (Lines 1546--1553).
    The structured type defines field \TLSlegacyVersion\ as constant 0x0303
    of aliased type \TLSProtocolVersion\ and field \TLSrandom\ of aliased
    type \TLSRandom, both of which are fixed length. The remaining fields
    are all variable length, for instance, \TLSlegacySessionId\ is a {0--32} 
    byte field of type \opaque. 
}]{listings/rfc8446.txt}
 

\lstinputlisting[
  float=tb,
  linerange={
    1695-1702
  },
  label=lst:ServerHello,
  caption={[\ServerHello\ specification]
    \ServerHello\ specification, which defines structured type \ServerHello.
    The structured type is similar to structured type \ClientHello, except
    \ClientHello\ fields \TLSlegacySessionId, \TLScipherSuites, and
    \TLSlegacyCompressionModes\ are replaced by fields \TLSlegacySessionIdEcho,
    \TLScipherSuite, and \TLSlegacyCompressionMode, respectively.
}]{listings/rfc8446.txt}


